Trees with proper thinness 2

The proper thinness of a graph is an invariant that generalizes the concept of a proper interval graph. Every graph has a numerical value of proper thinness and the graphs with proper thinness~1 are exactly the proper interval graphs. A graph is proper $k$-thin if its vertices can be ordered in such a way that there is a partition of the vertices into $k$ classes satisfying that for each triple of vertices $r < s < t$, such that there is an edge between $r$ and $t$, it is true that if $r$ and $s$ belong to the same class, then there is an edge between $s$ and $t$, and if $s$ and $t$ belong to the same class, then there is an edge between $r$ and $s$. The proper thinness is the smallest value of $k$ such that the graph is proper $k$-thin. In this work we focus on the calculation of proper thinness for trees. We characterize trees of proper thinness~2, both structurally and by their minimal forbidden induced subgraphs. The characterizations obtained lead to a polynomial-time recognition algorithm. We furthermore show why the structural results obtained for trees of proper thinness~2 cannot be straightforwardly generalized to trees of proper thinness~3.

==> src/intro.tex <==
Many optimization problems defined on graphs are computationally difficult. For these problems, it is natural to ask: \emph{For which subclasses of graphs can the problem be solved efficiently, and for which ones is it intrinsically difficult?}

Knowing that a family of graphs has a \emph{bounded width} (e.g., treewidth~\cite{R-S-minors2-tw} or clique-width~\cite{G-R-clique-width,C-O-cw-cographs}) has proven to be an extremely useful property for designing efficient algorithms, generally using dynamic programming, for many famous problems, such as the graph coloring problem or the maximum independent set problem~\cite{cygan2015parameterized}. Moreover, in many cases, very generally applicable algorithmic results, known as \emph{metatheorems}, have been achieved. A metatheorem has the form: \emph{``if a problem can be expressed in this particular language or with these kinds of restrictions: [corresponding type], then it can be solved in polynomial time for graphs of bounded [corresponding width]''}. Some examples of this can be found in~\cite{bodlaender1988, Cour-cw, C-M-cw-LinEMSOL, C-M-tree-MSOL}.

Since the 1980s, several width parameters on a graph have been defined, in order to encompass classes of graphs within which NP-complete problems will in general be polynomial.
In addition to those already mentioned, other examples of classical parameters are the \emph{path-width}~\cite{R-S-minors1-pw}, the \emph{bandwidth}~\cite{Pap-bandwidth,G-G-J-K-bandwidth}, and the \emph{boxicity}~\cite{Rob-box}. More recently, the \emph{thinness}~\cite{M-O-R-C-thinness}, the \textit{mim-width} and its linear version~\cite{VatshelleThesis}, the \emph{sim-width}~\cite{KANG20171} and in 2020 the \emph{twin-width}~\cite{BKTW20twinw} were incorporated. A quite powerful metatheorem for the mim-width~\cite{meta-mimw-arxiv} was recently announced.

\textbf{Thinness} was defined by Mannino, Oriolo, Ricci and Chandran in 2007 as part of an application to problems arising from cellular telephony related to the independent set problem~\cite{M-O-R-C-thinness}.

A graph $G = (V, E)$ is \emph{$k$-thin} if there exists an ordering of the vertices $v_1, v_2, \dots, v_n$ and a partition $V^1, \dots, V^k$ of $V$ into $k$ classes such that for every triple $(r, s, t)$ with $r < s < t$, if $v_r, v_s$ are in the same class and $v_t v_r \in E$, then $v_t v_s \in E$.

The minimum $k$ such that G is $k$-thin is called the thinness of $G$ and is denoted as $\thin(G)$. When an ordering and a partition satisfy the definition of $k$-thin, we say that the ordering and the partition are consistent. An example can be seen in Figure~\ref{fig:thinness}:

\begin{figure}[H]
\begin{center}
    \begin{tabular}{ccc}
\input{img/ejemplothinness.tex}  & \hspace{1cm} & \input{img/ejemploproperthinness.tex} \\
    \end{tabular}
\end{center}
\caption{A $3$-thin representation of a graph (left) and a proper $3$-thin representation of a graph (right). Vertices are ordered from bottom to top, and classes correspond to vertical lines.}\label{fig:thinness}
\end{figure}

The definition of thinness gave rise to the variants \emph{proper}~\cite{B-D-thinness}, \emph{independent or complete}~\cite{BGOSS-thin-oper}, \emph{precedence}~\cite{BOSS-thin-prec-dam-lagos}, \emph{mixed or inversion-free mixed} (and their own versions). These last variants were defined in 2022 by Balabán, Hlinený, and Jedelský~\cite{Mixed-thin-arxiv}, and they show that the parameter has attracted interest in the community in recent years. In particular, in ~\cite{B-D-thinness} a metatheorem-like result for thinness was obtained, i.e., it describes a large family of problems that can be solved in polynomial time on graphs of bounded thinness. Furthermore, the concept of \emph{proper thinness} is defined there and the family of problems that can be solved in polynomial time on graphs of bounded proper thinness is further extended, including domination problems.

A graph $G = (V, E)$ is \emph{proper $k$-thin} if there exists an ordering of the vertices $v_1, v_2, \dots, v_n$ and a partition $V^1, \dots, V^k$ of $V$ into $k$ classes such that for every triple $(r, s, t)$ with $r < s < t$ it holds that:
\begin{itemize}
\item If $v_r, v_s$ belong to the same class and $v_t v_r \in E$, then $v_t v_s \in E$
\item If $v_s, v_t$ belong to the same class and $v_t v_r \in E$, then $v_r v_s \in E$
\end{itemize}

The proper thinness of a graph $G$ is the smallest number $k$ for which the graph satisfies the definition of $k$-thin proper. It is denoted as $\pthin(G)$. When an ordering and a partition satisfy the definition of $k$-thin proper, we say that the ordering and partition are \emph{strongly consistent}. An example can be seen in Figure~\ref{fig:thinness}. 

% Well-known relationships between the more classical parameters and between some variants of thinness are shown in Figure~\ref{fig:map}. The relationship between thinness and other width parameters is obtained by combining results from~\cite{B-D-thinness,B-B-M-P-convex-wads,M-O-R-C-thinness}. Another recently shown relationship is that proper mixed $k$-thin graphs have linear twin-width in $k$~\cite{Mixed-thin-arxiv}, while interval (1-thin) graphs have unbounded twin-width~\cite{BKTW20twinw}.

% \input{img/diagramas-parametros.tex}

Regarding the recognition of thinness and proper thinness, it is proved in ~\cite{B-D-thinness,B-M-O-thin-tcs} that, given a vertex ordering, there is a cubic ordering algorithm that finds a (strongly) consistent partition into a minimal number of classes. However, given a vertex partitioning, it is NP-complete to decide whether there exists a (strongly) consistent ordering with that partition ~\cite{B-D-thinness}. In ~\cite{Shitov-thin}, reducing from that problem, it is shown that deciding whether a graph is $k$-thin is NP-complete. The complexity remains open for a fixed $k$ and for the proper variant.

Since computing thinness is NP-hard in general, the question is valid for restricted classes of graphs. It has been shown that computing thinness is polynomial for cographs~\cite{B-D-thinness} and for trees~\cite{Agus-Eric-ISCO22, Agus-Eric-tesis}. In both cases, the thinness can be arbitrarily large. The complexity of computing the proper thinness in both classes remains open.

The algorithm for tree thinness is inspired by the algorithm for linear mim-width of trees~\cite{Hogemo-trees-mimw}, which in turn is inspired by the algorithm for pathwidth of trees~\cite{E-S-T-pw-tree,Sch-pw-tree}.

It is known~\cite{B-D-thinness,M-O-R-C-thinness} that, in general,

$$\lmimw(G) \leq \thin(G) \leq \pw(G)+1.$$

On the other hand, in~\cite{B-B-lagos21-dam,Gaston-tesis}, it is proved that

$$\pthin(G) \leq \bw(G)+1.$$

However, it is not possible to draw inspiration from bandwidth algorithms in this case, since the problem is NP-complete even for certain fairly restricted subclasses of trees~\cite{Bw-cater} (the long-haired caterpillars with maximum degree~3). In fact, we will see that one of these subclasses of trees is properly contained in the trees with proper thinness of at most two.

From a structural point of view, a natural objective that arises is to achieve a characterization by forbidden induced subgraphs of the classes of graphs defined by their thinness or proper thinness. It is also valid to study it in particular for some classes of graphs.

A complete characterization by forbidden induced subgraphs is known for the thinness of cographs~\cite{B-D-thinness} and a structural characterization for the thinness of trees~\cite{Agus-Eric-tesis}. In both cases, the problem for proper thinness remains open.

In this work, we will address the study of both problems for the class of trees. From the above definitions, it follows that, for any graph, the inequality $\thin(G) \leq \pthin(G)$ holds. Since we know from~\cite{B-D-thinness} that the class of trees has no bounded thinness, then this class also has no bounded proper thinness.

Determining the proper thinness of a graph (in this case, a tree), and obtaining a strongly consistent ordering and partitioning is a useful problem because if the proper thinness in a graph is bounded, some NP-Complete problems can be solved in polynomial time, given the corresponding representation~\cite{B-D-thinness}.

\subsection{Definitions and Basic Properties}

All graphs in this work are finite, undirected, and have no loops or multiple edges.

Let $G$ be a graph, let $V(G)$ denote the set of its vertices or nodes and $E(G)$ the set of its edges. Let $N(v)$ denote the neighborhood of a vertex $v \in V$, that is, the set of vertices that are adjacent to $v$. Let $N[v]$ denote the closed neighborhood of a vertex $v \in V$, that is, $N(v) \cup \{ v \}$. If $X \in V(G)$, let $N(X)$ denote the set of vertices not in $X$ with at least one neighbor in $X$, and let $N[X]$ denote the closed neighborhood $N(X) \cup X$.

A graph $H$ is a \emph{subgraph} of a graph $G$ if $V(H) \subseteq V(G)$ and
$E(H) \subseteq E(G)$. Given a vertex set $W \subseteq V(G)$, the subgraph of
$G$ \emph{induced} by $W$ is the subgraph $H$ of $G$ such that $V(H) = W$ and $E(H)$ is the set of edges of $G$ that has both endpoints in $W$.

We denote the subgraph of $G$ induced by a set $W \subseteq V(G)$ by $G[W]$, and the graph $G[V(G) \setminus W]$ by $G - W$.

Two graphs $G$ and $H$ are \emph{isomorphic} if there exists a bijection between $V(G)$ and $V(H)$ that preserves adjacencies. In this case, we note $G = H$.

If $G_1$ and $G_2$ are two graphs, the disjoint union of $G_1$ and $G_2$, denoted by $G = G_1 \cup G_2$, is such that $V(G) = V_1 \cup V_2$, where $V_1$ and $V_2$ are disjoint, $G[V_1]$ is isomorphic to $G_1$, and $G[V_2]$ is isomorphic to $G_2$.

The \emph{degree} of a vertex $v$ in a graph $G$ is the number of edges that have $v$ as one of their endpoints, and is denoted by $d(v)$. A \emph{path} is an ordered list of vertices in which every vertex, except the first, is adjacent to the previous one. A \emph{simple path} is a path in which each vertex appears at most once.

An \emph{induced path} is a path such that there are no edges in the graph with both ends in the path that are not part of it (see example in Figure~\ref{fig:cam_ind}). When we say that a graph \emph{is a path}, we mean that all the vertices in the graph are part of an induced path.

%\input{img/caminos-inducidos.tex}

Two vertices are \emph{connected} in a graph $G$ if there exists a path that starts at one of the vertices and ends at the other. A connected graph is one in which all vertices are connected pairwise. A connected component or simply component of a graph $G$ is a maximal induced subgraph of $G$ that is connected.

The distance between two vertices $v$ and $w$ in a connected graph $G$ is the length of the shortest path between $v$ and $w$ (the length of a path is measured by the number of edges it comprises) and is denoted $d_G(v,w)$. If the context is unambiguous, it is abbreviated $d(v,w)$.

Given a graph $G$ and an edge $uv \in E(G)$, the graph obtained by the \emph{subdivision} of the edge $uv$ is the graph $G'$
such that $V(G') = V(G) \cup \{w\}$ ($w \not \in V(G)$) and $E(G') = E(G) \setminus \{uv\} \cup \{uw,wv\}$. That is, the edge $uv$ is converted into a path of length two with endpoints $u$ and $v$. A graph $H$ is said to be \emph{a subdivision} of the graph $G$ if $H$ can be obtained from $G$ by applying a finite number of edge subdivisions. A \emph{cycle} is a path with at least four vertices in which the first and last vertices are equal and no other vertices are repeated. A \emph{tree} is a connected graph with no cycles. A \emph{leaf} of a tree $T$ is a vertex of $T$ with degree one.

A tree $T$ is a \emph{caterpillar} if it contains an induced path $P$ such that $V(T) = N[P]$. A \emph{long-haired caterpillar} is a subdivision of a caterpillar.

A \emph{forest} is a graph with no cycles, that is, a graph such that each of its connected components is a tree. Equivalently, a forest is the disjoint union of trees.

A graph $H$ is a \emph{forbidden subgraph} for a given class of graphs if a graph in that class cannot contain $H$ as an induced subgraph. The forbidden subgraph is \emph{minimal} if any induced subgraph proper to it belongs to the class.

Consider a finite family of nonempty sets. The \emph{intersection graph}
of this family is obtained by representing each set by a vertex and connecting two vertices by an edge if and only if the corresponding sets intersect. It is
simple to prove that every graph is the intersection graph of some family. It then makes sense to study particular families.

An \emph{interval graph} is the intersection graph of intervals on a line. Thinness is the generalization of interval graphs:

\begin{theorem}\emph{\cite{Ola-interval,R-PR-interval}}
A graph $G = (V, E)$ is an interval graph if there exists an ordering of the vertices $v_1, v_2, \dots, v_n$ such that for every triple $(r, s, t)$ with $r < s < t$, if $v_t v_r \in E$, then $v_t v_s \in E$.
\end{theorem}

In turn, proper thinness is the generalization of proper interval graphs, which are interval graphs that admit an intersection model in which no interval is properly contained in another.

\begin{theorem}\emph{\cite{Rob-uig}}
A graph $G = (V, E)$ is a proper interval graph if there exists an ordering of the vertices $v_1, v_2, \dots, v_n$ such that for every triple $(r, s, t)$ with $r < s < t$, if $v_t v_r \in E$, then $v_t v_s \in E$ and $v_r v_s \in E$.
\end{theorem}

Note that these characterizations correspond, respectively, to the definitions of thinness and proper thinness for the case $k=1$, that is, all vertices in the same class. This implies that interval graphs and 1-thin graphs are the same class, and proper interval graphs and 1-thin graphs are the same class.

Interval graphs, and therefore thinness~1 graphs, can be recognized in polynomial time~\cite{B-L-PQtrees} and were characterized by forbidden induced subgraphs~\cite{L-B-interval-AT}. \begin{figure}
\begin{center} 
\epsfig{file=img/lagos1.eps}\quad\epsfig{file=img/lagos6.eps}\quad\epsfig{file=img/lagos21.eps} 
\quad\epsfig{file=img/lagos23.eps}\quad\epsfig{file=img/lagos24.eps}
\caption{Minimal forbidden induced subgraphs for the class of interval graphs.}\label{fig:LekkerkerkerBoland}
\end{center}
\end{figure}

\begin{theorem}\emph{\cite{L-B-interval-AT}}\label{th:LekkerkerkerBoland}
The minimal forbidden induced subgraphs for the class of interval graphs are: bipartite claw, $n$-net for $n\geq 2$, umbrella,
$n$-tent for $n\geq 3$, and $C_n$ for $n\geq 4$ (Figure~\ref{fig:LekkerkerkerBoland}).\\
\end{theorem}

Proper interval graphs, and therefore proper thinness graphs~1, can also be recognized in polynomial time~\cite{F-M-M-prop-int} and were characterized by forbidden induced subgraphs~\cite{Rob-uig}.

\begin{theorem}\emph{\cite{Rob-uig}}\label{th:Roberts}
A graph is a proper interval graph if and only if it is an interval graph and does not have the claw as an induced subgraph (Figure~\ref{fig:proh-intp}). Equivalently, the minimal forbidden induced subgraphs for the class of proper interval graphs are: claw, net, tent, and $C_n$ for $n\geq 4$ (Figure~\ref{fig:Roberts}).\\
\end{theorem}

\input{img/proh-int-prop}

==> src/pthin2.tex <==
\subsection{Interval and proper interval trees and forests}

It is easy to see that every caterpillar is an interval graph. Furthermore, the graph in Figure~\ref{fig:proh-int} is known to be one of the minimal forbidden induced subgraphs for the class of interval graphs~\cite{L-B-interval-AT}. Therefore, interval trees are exactly the caterpillars, and interval forests turn out to be the disjoint union of caterpillars.

\input{img/proh-int.tex}

In turn, the graph in Figure~\ref{fig:proh-intp}, known as \emph{claw} or $K_{1,3}$, is known to be the only minimal forbidden induced subgraph for the class of proper interval graphs, within the class of interval graphs~\cite{Rob-uig}. Therefore, proper interval trees are just paths, and proper interval forests turn out to be the disjoint union of paths.

Thus, in the partition of a thin representation of a graph, each of the classes is a disjoint union of caterpillars, and for a proper thin representation, a disjoint union of paths.

\subsection{Structural Characterization}

In \cite{Agus-Eric-ISCO22,Agus-Eric-tesis}, it was shown that the following result is valid for the thinness of trees: Given a tree $T$ with thinness equal to $k$, one can always obtain a simple path $C$ such that all the connected components of $T - N[C]$ have thinness less than $k$, and furthermore, the vertices of $N[C]$ form one of the classes of a $k$-thin partition of $T$.

In this work, we attempt to obtain a similar result for the proper thinness of trees. In this case, taking a simple path $C$ in $T$ and observing the proper thinness of the connected components of $T - C$. We will show that this result is valid for the case of trees of proper thinness 2, that is, there always exists a simple path $C$ such that one can take a partition (which is strongly consistent with some ordering) into two classes: one with the vertices of $C$ and another with the vertices of $T - C$.

\subsubsection{Structural Characterization Theorem}

The main result of this work is the following.

\begin{theorem}\label{theorem:characterization_pthin2_pt2}
A tree T has pthin(T) = 2 if and only if the following hold simultaneously:
    \begin{enumerate}
        \item There exists some vertex in T with degree greater than or equal to 3.
        \item If v is a vertex of T with degree greater than or equal to 5, then at most 4 of its neighbors have degree greater than 1.
        \item There exists a simple path $C_0$ in T such that:
        \begin{enumerate}
            \item All vertices of T with degree greater than or equal to 4 are in $C_0$.
            \item If some vertex v of degree 3 is not in $C_0$, then:
            \begin{enumerate}
                \item v is adjacent to a vertex w of $C_0$.
                \item The degree of w is less than or equal to 3. 
            \end{enumerate} 
        \end{enumerate} 
    \end{enumerate}
\end{theorem}

The following corollaries follow from the previous theorem:

\begin{corollary}\label{coro:pthin2_connected_class_pt2}
Let $T = (V, E)$ be a tree such that $pthin(T) = 2$. Then, there exists a simple path $C_0 = v_1, \dots, v_k$ in $T$ such that there exists an ordering that is strongly consistent with the partition with the class partition $S = \{ V^0, V^1 \}$, where $V^0 = \{ v_1, \dots, v_k \}$ and $V^1 = V - V^0$.
\end{corollary}

\begin{corollary}\label{coro:pthin2_subtreespthin1_pt2}
Let $T = (V, E)$ be a tree such that pthin(T) = 2. Then, there exists a simple path $C_0$ such that all connected components of $T - C_0$ have proper thinness equal to~1.
\end{corollary}

\subsection{Characterization by minimal forbidden induced subgraphs}

From the Theorem \ref{theorem:characterization_pthin2}, we also obtained a characterization by minimal forbidden induced subgraphs:

\input{img/forbidden_pt2.tex}

\begin{theorem}\label{theorem:forbidden_subtrees_pt2}
    Let $T$ be a tree. Then, pthin(T)=2 if and only if $T$ does not contain any of the trees in Figure~\ref{fig:prohibidos_pt2} as an induced subgraph and $T$ has at least one vertex of degree greater than or equal to~3.
\end{theorem}

\begin{proposition} 
The graphs in Figure~\ref{fig:prohibidos_pt2} are minimal.
\end{proposition}

\begin{proposition}\label{prop:pthin2_degree_5_pt2}
Let $T$ be a tree such that pthin($T$) = 2. If $v$ is a vertex of $T$ with degree greater than or equal to~5, then at most~4 of its neighbors have degree greater than~1.
\end{proposition}

\begin{proof}
Let v be a vertex of $T$ with $d(v) \geq 5$. By Proposition \ref{prop:same_class_neighbors}, there are at most two vertices of $N(v)$ in the same class as $v$. Let $v_1 < \dots < v_l$ be the vertices neighboring $v$ in the other class. By Proposition \ref{prop:neighbors_another_class}, of all such vertices, only $v_1$ and $v_l$ can have degree greater than~1.
\end{proof}

\begin{proposition}\label{prop:pthin2_has_path_pt2}
Let T be a tree such that pthin(T) = 2. Then, there exists a simple path $C_0$ in T such that:
\begin{enumerate}
\item All vertices of T with degree greater than or equal to 4 are in $C_0$.
\item If any vertex v of degree 3 is not in $C_0$, then:
\begin{enumerate}
\item v is adjacent to a vertex w in $C_0$.
\item The degree of w is less than or equal to 3.
\end{enumerate}
\end{enumerate}
\end{proposition}

==> src/pthin3.tex <==
\subsection{Results to generalize}

We know that for the case of trees with proper thinness equal to 2, the Corollaries \ref{coro:pthin2_connected_class} and \ref{coro:pthin2_subtreespthin1} are valid.

We would like to see if this can be generalized to the case of trees with proper thinness greater than 2, that is, to see if it can be true, given a tree with proper thinness equal to $n$ (with $n > 2$):
\begin{itemize}
\item That, given a partition into $n$ classes and a strongly consistent ordering, there exists a simple path such that that path can be one of the classes of the partition.
\item Or, that there exists a simple path such that, by removing the vertices from that path, the connected components of the resulting subgraph have strictly smaller proper thinness.
\end{itemize}

\section{Counterexample}

However, neither of these statements are true for trees with proper thinness equal to 3. This can be proven using the counterexample $T_A$, which consists of three copies of the tree $T_0$ from Theorem \ref{theorem:forbidden_subtrees}, joined by a vertex we call $v_0$.

\input{img/counterexample_base.tex}

\begin{proposition}
$T_A$ has proper thinness equal to 3.
\end{proposition}

\begin{proof}
To prove that $pthin(T_A) \leq 3$, we show a proper $3-thin$ representation of $T_A$. The vertices are ordered from bottom to top, and the classes correspond to the vertical lines.

\input{img/counterexample_representation.tex}

Furthermore, since $T_A$ has as a subtree the graph $T_0$ of Theorem \ref{theorem:forbidden_subtrees}, we know that $pthin(T_A) \geq 3$.
\end{proof}

\begin{remark}\label{obs:one_in-each_class}
Since $T_A$ consists of three copies of $T_0$ joined by vertex $v_0$, and we already proved that it has $pthin(T_0) = 3$, then, given $S = \{ V^0, V^1, V^2 \}$ a class partition of the vertices of $T_A$ and $\sigma$ an ordering of the vertices such that $S$ and $\sigma$ are strongly consistent, each of those three subtrees has at least one vertex in each of the three classes.
\end{remark}

\begin{proposition}
Let $S = \{V^0, V^1, V^2\}$ be a class partition of the vertices of $T_A$ and let $\sigma$ be an ordering of the vertices such that $S$ and $\sigma$ are strongly consistent. Then, the induced subgraphs $T_A[V^0]$, $T_A[V^1]$ and $T_A[V^2]$ are not connected.
\end{proposition}

\begin{proposition}
Let $C_0$ be a simple path of $T_A$. Then, the subgraph $T - C_0$ has proper thinness equal to 3.
\end{proposition}

\subsection{Valid results for trees of proper thinness 3}

Therefore, with the previous counterexample, we show that for trees of proper thinness 3, the following two results are valid:

\begin{proposition}\label{prop:path1}
Let $T = (V, E)$ be a tree such that $pthin(T) = 3$. Then, there does not necessarily exist a simple path $C_0 = v_1, \dots, v_k$ in $T$ such that there exists an ordering that is strongly consistent with the partition with the class partition $S = \{V^0, V^1, V^2 \}$ (where $V^0 = \{v_1, \dots, v_k \}$).
\end{proposition}

\begin{proposition}\label{prop:path2}
Let $T = (V, E)$ be a tree such that $pthin(T) = 3$. Then, there does not necessarily exist a simple path $C_0 = v_1, \dots, v_k$ in $T$ such that all connected components of $T - C_0$ have proper thinness less than 3.
\end{proposition}
